Energy absorption in the laser-QED regime

A theoretical and numerical investigation of non-ponderomotive absorption at laser intensities relevant to quantum electrodynamics is presented. It is predicted that there is a regime change in the dependence of fast electron energy on incident laser energy that coincides with the onset of pair production via the Breit-Wheeler process. This prediction is numerically verified via an extensive campaign of QED-inclusive particle-in-cell simulations. The dramatic nature of the power law shift leads to the conclusion that this process is a candidate for an unambiguous signature that future experiments on multi-petawatt laser facilities have truly entered the QED regime.

==> ZVPQEDbib.tex <==
@article{BaevaZVP,
  author = "T. Baeva and S. Gordienko and A.P.L. Robinson and P.A. Norreys",
  title = "The zero vector potential mechanism of attosecond absorption",
  journal = "Phys. Plasma",
  volume = "18",
  pages = "056702",
  year = "2011"
}

@article{SavinZVP,
    author = "A. F. Savin and A. J. Ross and M. Serzans and R. M. G. M. Trines and L. Ceurvorst and N. Ratan and B. Spiers and R. Bingham and A. P. L. Robinson and P. A. Norreys",
    title = "Attosecond-scale absorption at extreme intensities",
    journal = "Phys. Plasma",
    volume = "24",
    pages = "113103",
    year = "2017"
}

@article{WilksPond,
  author = "S. C. Wilks and W. L. Kruer",
  title = "Absorption of {U}trashort, {U}ltra-intense {L}aser {L}ight by {S}olids and {O}verdense {P}lasmas",
  journal = "IEEE J Quantum Elect.",
  volume = "33",
  pages = "1954",
  year = "1997"
}

@article{BrunelHeating,
  author = "F. Brunel",
  title = "Not-{S}o-{R}esonant, {R}esonant {A}bsorption",
  journal = "Phys. Rev. Lett.",
  volume = "59",
  pages = "52",
  year = "1987"
}

@article{ForslundAnharmonicResonance,
  author = "W. Forslund and J. M. Kindel and K. Lee",
  title = "Theory of {H}ot {E}lectron {S}pectra at {H}igh {L}aser {I}ntensity",
  journal = "Phys. Rev. Lett.",
  volume = "39",
  pages = "284",
  year = "1977"
}

@article{MulserAnharmonicResonance,
  author = "P. Mulser and D. Bauer and H. Ruhl",
  title = "Collisionless {L}aser-{E}nergy {C}onversion by {A}nharmonic {R}esonance",
  journal = "Phys. Rev. Lett.",
  volume = "101",
  pages = "225002",
  year = "2008"
}

@article{GibbonVacuum,
  author = "P. Gibbon and A. R. Bell",
  title = "Collisionless {A}bsorption in {S}harp-{E}dged {P}lasmas",
  journal = "Phys. Rev. Lett.",
  volume = "68",
  pages = "1535",
  year = "1992"
}

@article{GordienkoRelSim,
  author = "S. Gordienko and A. Pukhov",
  title = "Scalings for ultrarelativistic laser plasmas and quasimonoenergetic electrons",
  journal = "Phys. Plasmas",
  volume = "12",
  pages = "043109",
  year = "2005"
}

@article{TeubnerHHG,
  author = "U. Teubner and P. Gibbon",
  title = "High-order harmonics from laser-irradiated plasma surfaces",
  journal = "Rev. Mod. Phys.",
  volume = "81",
  pages = "445",
  year = "2005"
}

@article{FonsecaOSIRIS,
  author = "R. A. Fonseca and L. O. Silva and F. S. Tsung and V. K. Decyk and W. Lu and C. Ren and W. B. Mori and S. Den and S. Lee and T. Katsouleas and J. C. Adam",
  title = "{OSIRIS}: {A} three-dimensional, fully relativistic particle in cell code for modelling plasma based accelerators",
  journal = "Lect. Notes. Comp. Sci.",
  volume = "2231",
  pages = "342",
  year = "2002"
}

@article{ThauryMirror,
  author = "C. Thaury and F. Qu\'er\'e and J.-P. Geindre and A. Levy and T. Ceccotti and P. Monot and > Bougeard and F. R\'eau and P. D'Oliveira and P. Audebert and R. Marjoribanks and Ph. Martin",
  title = "Plasma mirrors for ultrahigh-intensity optics",
  journal = "Nat. Phys.",
  volume = "3",
  pages = "424",
  year = "2007"
}

@article{VincentiMirror,
  author = "H. Vincenti and S. Monchoc\'e and S. Kahaly and G. Bonnaud and Ph. Martin and F. Qu\'er\'e",
  title = "Optical properties of relativistic plasma mirrors",
  journal = "Nat. Commun.",
  volume = "5",
  year = "2014"
}

@article{BaevaHHG,
  author = "T. Baeva and S. Gordienko and A. Pukhov",
  title = "Theory of high-order harmonic generation in relativistic laser interaction with over-dense plasma",
  journal = "Phys. Rev. E",
  volume = "74",
  pages = "046404",
  year = "2006"
}
  
 @book{SteaneHeadlight,
   author = "A. M. Steane",
   title = "Relativity made relatively easy",
   publisher = "OUP, United Kingdom",
   pages = "44--50",
   year = "2012"
 }

@book{Steane4vectors,
   author = "A. M. Steane",
   title = "Relativity made relatively easy",
   publisher = "OUP, United Kingdom",
   pages = "32--39",
   year = "2012"
 }

@article{ZepfScalelength,
  author = "M. Zepf and G. D. Tsakiris and G. Pretzler and I. Watts and D. M. Chambers and P. A. Norreys and U. Andiel and A. E. Dangor and K. Eidmann and C. Gahn and A. Machacek and J. S. Wark and K. Witte",
  title = "Role of the plasma scale length in the harmonic generation from solid targets",
  journal = "Phys. Rev. E",
  volume = "5",
  pages = "R5253",
  year = "1998"
}

@article{TarasevitchScalelength,
  author = "A. Tarasevitch and A. Orisch and D. {Von Der Linde} and Ph. Balcou and G. Rey and J.-P. Chambaret and U. Teubner and D. Kl{\"o}pfel and W. Theobald",
  title = "Generation of high-order spatially coherent harmonics from solid targets by femtosecond laser pulses!",
  journal = "Phys. Rev. A",
  volume = "62",
  pages = "1",
  year = "2000"
}

 @book{Chencritden,
   author = "F. F. Chen",
   title = "Introduction to plasma physics and controlled fusion {V}olume 1: {P}lasma {P}hysics",
   publisher = "Plenum Press, United States of America",
   pages = "114--120",
   year = "1984"
 } 
 
 @article{DromeyExp1,
   author = "B. Dromey and M. Zepf and A. Gopal and K. Lancaster and M. S. Wei and K. Krushelnick and M. Tatarakis and N. Vakakis and S. Moutaizis and R. Kodama and M. Tampo and C. Stoeckl and R. Clarke and H. Habara and D. Neely and S. Karsch and P. A. Norreys",
   title = "High harmonic generation in the relativistic limit",
   journal = "Nat. Phys.",
   volume = "2",
   pages = "456",
   year = "2006"
 }
 
 @article{DromeyExp2,
   author = "B. Dromey and S. Kar and C. Bellei and D. C. Carroll and R. J. Clarke and J. S. Green and S. Kneip and K. Markey and S. R. Nagel and P. T. Simpson and L. Willingale and P. McKenna and D. Neely and Z. Najmudin and K. Krushelnick and P. A. Norreys and M. Zepf",
   title = "Bright multi-ke{V} harmonic generation from relativistically oscillating plasma surfaces",
   journal = "Phys. Rev. Lett",
   volume = "99",
   pages = "115003",
   year = "2007"
 }
 
 @article{SadlerXFEL,
   author = "J. Sadler and R. Nathvani and P. Ole\'skiewicz and L. Ceurvorst and N. Ratan and M. F. Kasim and R. M. G. M. Trines and R. Bingham and P. A. Norreys",
   title = "Compression of {X}-ray free electron laser pulses to attosecond duration",
   journal = "Sci. Rep.",
   volume = "5",
   pages = "16755",
   year = "2015"
}

@article{KrauszAttosecond,
    author = "F. Krausz and M. Ivanov",
    title = "Attosecond physics",
    journal = "Rev. Mod. Phys.",
    volume = "81",
    pages = "163",
    year = "2009"
}

@article{NeutzeNature,
    author = "R. Neutze and R. Wouts and D. {Van der Spoel} and E. Weckert and J. Hajdu",
    title = "Potential for biomolecular imaging with femtosecond {X}-ray pulses",
    journal = "Nature",
    volume = "406",
    pages = "752",
    year = "2000"
}

@article{LiHosing,
    author = "G. Li and R. Yan and C. Ren",
    title = "Laser {C}hanneling in {M}illimeter-Scale {U}nderdense {P}lasmas of {F}ast-{I}gnition {T}argets",
    journal = "Phys. Rev. Lett.",
    volume = "100",
    pages = "125002",
    year = "2008"
}

@article{SarriHosing,
    author = "G. Sarri and K. L. Lancaster and R. Trines and E. L. Clark and S. Hassan and J. Jiang and N. Kageiwa and N. Lopes and R. Ramis and A. Rehman and X. Ribeyre and C. Russo and R. H. H. Scott and T. Tanimoto and M. Temporal and M. Borghesi and J.R. Davies and Z. Najmudin and K. A. Tanaka and M. Tatarakis and P. A. Norreys",
    title = "Creation of persistent, straight, 2 mm long laser driven channels in underdense plasmas",
    journal = "Phys. Plasmas",
    volume = "17",
    pages = "113303",
    year = "2010"
}

@article{NajmudinHosing,
    author = "Z. Najmudin and K. Krushelnick and M. Tatarakis and E.L. Clark and C. N. Danson and V. Malka and D. Neely and M. I. K. Santala and A.E. Dangor",
    title = "The effect of high intensity laser propagation instabilities on channel formation in underdense plasmas",
    journal = "Phys. Plasmas",
    volume = "10",
    pages = "438",
    year = "2003"
}

@article{ChenHosing,
    author = "L. M. Chen and H. Kotaki and K. Nakajima and J. Koga and S. V. Bulanov and T. Tajima and Y. Q. Gu and H. S. Peng and X. X. Wang and T. S. Wen and H. J. Liu and C. Y. Jiao and C. G. Zhang and X. J. Huang and Y. Guo and K. N. Zhou and J. F. Hua and W. M. An and C. X. Tang and Y. Z. Lin",
    title = "Self-guiding of 100 {TW} femtosecond laser pulses in centimeter-scale underdense plasma",
    journal = "Phys. Plasmas",
    volume = "14",
    pages = "040703",
    year = "2007"
}

@article{CeurvorstHosing,
    author = "L. Ceurvorst and N. Ratan and M. C. Levy and M. F. Kasim and J. Sadler and R. H. H. Scott and R. M. G. M. Trines and T. W. Huang and M. Skramic and M. Vranic and L. O. Silva and P. A. Norreys",
    title = "Mitigating the hosing instability in relativistic laser-plasma interactions",
    journal = "N. J. Phys.",
    volume = "18",
    pages = "053023",
    year = "2016"
}

@article{WilksIntense,
    author = "S. C. Wilks and W. L. Kruer and M. Tabak and A. B. Langdon",
    title = "Absorption of ultra-intense laser pulses",
    journal = "Phys. Rev. Lett.",
    volume = "69",
    pages = "1383",
    year = "1992"
}

@article{DollarScalelength,
    author = "F. Dollar and P. Cummings and V. Chvykov and L. Willingale and M. Vargas and V. Yanovksy and C. Zulick and A. Maksimchuk and A. G. R. Thomas and K. Krushelnick",
    title = "Scaling high-order harmonic generation from laser-solid interactions to ultrahigh intensity",
    journal = "Phys. Rev. Lett.",
    volume = "110",
    pages = "175002",
    year = "2013"
}

@article{TajimaELI,
    author = "T. Tajima",
    title = "Prospect for extreme field science",
    journal = "Eur. Phys. J. D",
    volume = "55",
    pages = "519",
    year = "2006"
}

@article{MourouELI,
    author = "G. A. Mourou and C. L. Labaune and M. Dunne and N. Naumova and V. T. Tikhonchuk",
    title = "Relativistic laser-matter interaction: from attosecond pulse generation to fast ignition",
    journal = "Plasma Phys. Contr. F.",
    volume = "49",
    pages = "B667",
    year = "2007"
}

@article{ZouApollon,
    author = "J.P. Zou and C. Le{B}lanc and D. N. Papadopoulos and G. Ch\'eriaux and P. Georges and G. Mennerat and F. Druon and L. Lecherbourg and A. Pellegrina and P. Ramirez and F. Giambruno and A. Fr'eneaux and G. Leconte and D. Badarau and J. M. Boudenne and D. Fournet and T. Valloton and J. L. Paillard and j. L. Veray and M. Pina and P. Monot and J. P. Chambaret and P. Martin and F. Mathieu and P. Audebert and F. Amiranoff",
    title = "Design and current progress of the {A}pollon {10 PW} project",
    journal = "High Power Lasr Science and Engineering",
    Volume = "3",
    pages = "e2",
    year = "2015"
}

@article{BellPairProduction,
    author = "A.R. Bell and J. G. Kirk",
    title = "Possibility of {P}rolific {P}air {P}roduction with {H}igh-{P}ower {L}asers",
    journal = "Phys. Rev. Lett.",
    volume = "101",
    pages = "200403",
    year = "2008"
}

@article{MartinsLWFA,
    author = "S. F. Martins and J. Vieira and F. Fiuza and R. A. fonseca and C. Huang and W. Lu and W. B. Mori and R. Trines and P. Norreys and L. O. Silva",
    title = "Numerical simulations of {LWFA} for the next generation of laser systems",
    journal = "Advanced Accelerator Concepts",
    volume = "1086",
    pages = "285",
    year = "2009"
}

@article{RobinsonRPA,
    author = "A. P. L. Robinson and M. Zepf and S. Kar and R. G. Evans and C. Bellei",
    title = "Radiation pressure acceleration of thing foils with circularly polarized laser pulses",
    journal = "New J. Phys.",
    volume = "10",
    pages = "013021",
    year = "2008"
}

@article{NaumovaHoleBoring,
    author = "N. Naumova and T. Schlegel and V. T. Tikhonchuk and C. Labaune and I. V. Sokolov and G. Mourou",
    title = "Hole boring in a {DT} {P}ellet and {F}ast-{I}on {I}gnition with {U}ltraintense {L}aser {P}ulses",
    journal = "Phys. Rev. Lett.",
    volume = "102",
    pages = "025002",
    year = "2009"
}

@article{GordienkoFocusHHG,
    author = "S. Gordienko and A. Pukhov and O. Shorokhov and T. Baeva and T. Gordienko",
    title = "Coherent focusing of high harmonics: {A} new way towards the extreme intensities",
    journal = "Phys. Rev. Lett.",
    volume = "94",
    pages = "103903",
    year = "2005"
}

@book{DavisLaserBook,
    author = "C. C. Davis",
    title = "Lasers and {E}lectro-{O}ptics - {F}undamentals and {E}ngineering",
    publisher = "CUP",
    pages = "348 -- 354",
    year = "1996"
}

@article{LiWaterWindow,
    author = "J. Li and X. Ren and Y. Yin and K. Zhao and A. Chew and Y. Cheng and E. Cunningham and Y. Wang and S. Hu and Y. Wu and M. Chini and Z. Chang",
    title = "53-attosecond {X}-ray pulses reach the carbon {K}-edge",
    journal = "Nature Communications",
    volume = "8",
    pages = "186",
    year = "2017"
}

@article{FernandezIonIgnition,
	author = "J. C. Fern\'{a}ndez and others",
	title = "Progress and prospects of ion-driven fast ignition",
	journal = "Nucl. Fusion",
	year = "2009"
}

@article{PatelIsochoricHeating,
	author = "P. K. Patel and others",
	title = "Isochoric {H}eating of {S}olid-{D}ensity {M}atter with an {U}ltrafast {P}roton {B}eam",
	journal = "Phys. Rev. Lett.",
	year = "2003"
}

@article{DyerOpacityMeasurements,
	author = "R. Dyer and others",
	title = "	Single-shot time resolved expansion and emission measurements of proton-heated warm dense matter",
	journal = "Conference on {L}asers and {E}lectro-{O}ptics, 2007, {CLEO} 2007",
	year = "2007"
}

@article{LorenzEOSMeasurements,
	author = "K. T. Lorenz and others",
	title = "High pressure, quasi-isentropic compression experiments on the {O}mega laser",
	journal = "High Energy Density Physics",
	year = "2006"
}

@article{YogoMVA,
	author = "A. Yogo and others",
	title = "Laser ion acceleration via control of the near-critical density target",
	journal = "Phys. Rev. E",
	volume = "77",
	pages = "016401",
	year = "2008"
}

@article{BulanovMVA,
	author = "S. S. Bulanov and others",
	title = "Generation of {GeV} protons from 1 {PW} laser interaction with near critical density targets",
	journal = "Phys. Plasma",
	year = "2010"
}

@article{FukudaMVA,
	author = "Y. Fukuda others",
	title = "Energy {I}ncrease in {M}ulti-{MeV} {I}on {A}cceleration in the {I}nteraction of a {S}hort {P}ulse {L}aser with a {C}luster-{G}as {T}arget",
	journal = "Phys. Rev. Lett.",
	year = "2009"	
}

@article{NakamuraMVA,
	author = "T. Nakamura and others",
	title = "High-{E}nergy {I}ons from {N}ear-{C}ritical {D}ensity {P}lasmas via {M}agnetic {V}ortex {A}cceleration",
	journal = "Phys. Rev. Lett.",
	year = "2010"
}

@article{SnaveleyTNSA,
	author = "R. A. Snavely and others",
	title = "Intense {H}igh-{E}nergy {P}roton {B}eams from {P}etawatt-{L}aser {I}rradiation of {S}olids",
	journal = "Phys. Rev. Lett.",
	volume = "85",
	pages = "2945--2948",
	year = "2000"
}

@article{WilksTNSA,
	author = "S. C. Wilks and others",
	title = "Energetic proton generation in ultra-intense laser-solid interactions",
	journal = "Phys. Plasmas",
	volume = "8",
	pages = "542",
	year = "2001"
}

@article{CeccotiTNSA,
	author = "T. Ceccotti and others",
	title = "Proton {A}cceleration with {H}igh-{I}ntensity {U}ltrahigh-{C}ontrast {L}aser {P}ulses",
	journal = "Phys. Rev. Lett.",
	year = "2007"
}

@article{CrowTNSA,
	author = "J. E. Crow and P. L. Auer and J. E. Allen",
	title = "The expansion of a plasma into a vacuum",
	journal = "J. Plasma Physics",
	year  ="1975"	
}

@article{FuchsTNSA,
	author = "J. Fuchs and others",
	title = "Laser-driven proton scaling laws and new paths towards energy increase",
	journal = "Nature Physics",
	year = "2005"
}

@article{HatchettTNSA,
	author = "S. P. Hatchett and others",
	title = "Electron, photon, and ion beams from the relativistic interaction of {P}etawatt laser pulses with solid targets",
	journal = "Phys. Plasmas",
	year = "2000"
}

@article{MaksimchukTNSA,
	author = "A. Maksimchuk and others",
	title = "Forward {I}on {A}cceleration in {T}hin {F}ilms {D}riven by a {H}igh-{I}ntensity {L}aser",
	journal = "Phys. Rev. Lett.",
	year = "2000"
}

@article{EsirkepepovRPA,
	author = "T. Esirkepov and others",
	title = "Highly {E}fficient {R}elativistic-{I}on {G}eneration in the {L}aser-{P}iston {R}egime",
	journal = "Phys. Rev. Lett.",
	year = "2004"
}

@article{HenigRPA,
	author = "A. Henig and others",
	title = "Radiation-{P}ressure {A}cceleration of {I}on {B}eams {D}riven by {C}ircularly {P}olarized {L}aser {P}ulses",
	journal = "Phys. Rev. Lett.",
	volume = "103",
	pages = "245003",
	year = "2009"
}

@article{KarRPA,
	author = "S. Kar and others",
	title = "Ion {A}cceleration in {M}ultispecies {T}argets {D}riven by {I}ntense {L}aser {R}adiation {P}ressure",
	journal = "Phys. Rev. Lett.",
	year = "2012"
}

@article{FiuzaCSA,
	author = "F. Fiuza and others",
	title = "Laser-{D}riven {S}hocl {A}cceleration of {M}onoenergetic {I}on {B}eams",
	journal = "Phys. Rev. Lett.",
	volume = "109",
	pages = "215001",
	year = "2012"
}

@article{HaberbergerCSA,
	author = "D. Haberberger and others",
	title = "Collisionless shocks in laser-produced plasma generate monoenergetic high-energy proton beams",
	journal = "Nature Physics",
	year = "2011"
}

@article{HenigBOA,
	author = "A. Henig and others",
	title = "Enhanced Laser-{D}riven {A}cceleration in the {R}elativstic {T}ransparency {R}egime",
	journal = "Phys. Rev. Lett.",
	volume = "103",
	pages = "045002",
	year = "2009"
}

@article{YinBOA,
	author = "L. Yin and others",
	title = "Three-{D}imensional {D}ynamics of {B}reakout {A}fterburner {I}on {A}cceleration {U}sing {H}igh-{C}ontrast {S}hort-{P}ulse {L}aser and {N}anoscale {T}argets",
	journal = "Phys. Rev. Lett.",
	year = "2011"
}

@article{Cairns1,
	author = "R. A. Cairns and others",
	title = "Laminar shocks in high power laser plasma interactions",
	journal = "Phys. Plasmas",
	year = "2014"
}

@article{Cairns2,
	author = "R. A. Cairns and others",
	title = "Weak collisionless shocks in laser-plasmas",
	journal = "Plasma Phys. Control. Fusion",
	year = "2015"
}

@article{MusgraveVulcan,
	author = "I. Musgrave and others",
	title = "Review of laser diagnostics at the {V}ulcan laser facility",
	journal = "High Power Laser Science and Engineering",
	year = "2015"
}

@article{HoppsOrion,
	author = "N. Hopps and others",
	title = "Comprehensive descritpion of the {O}rion laser facility",
	journal = "Plasma Phys. Control. Fusion",
	year = "2015"
}

@article{KogaQEDThomson,
	author = "J. Koga and T. Zh. Esirkepov and S. V. Bulanov",
	title = "Nonlinear {T}homson scattering with strong radiation damping",
	journal = "J. Plasma Phys.",
	year = "2006"
}

@article{MullerQEDLaser,
	author = "C. M{\"{u}}ller others",
	title = "Relativistic {N}onperturbative {A}bove-{T}hreshold {P}henomena in {S}trong {L}aser {F}ields",
	journal = "Laser Physics",
	year = "2009"
}

@article{HawkingHawkingRadiation,
	author = "S. W. Hawking",
	title = "Black hole explosions?",
	journal = "Nature",
	year = "1974"
}

@article{FullingUnruhEffect,
	author = "S. A. Fulling",
	title = "Nonuniqueness of {C}anonical {F}ield {Q}uantization in {R}iemannian {S}pace-{T}ime",
	journal = "Phys. Rev. D",
	year = "1973"
}

@article{DaviesUnruhEffect,
	author = "P. C. W. Davies",
	title = "Scalar production in the {S}chwarzschild and {R}indler metrics",
	journal = "J. Phys. A",
	year = "1975"
}

@article{UnruhUnruhEffect,
	author = "W. G. Unruh",
	title = "Notes on black-hole evaporation",
	journal = "Phys. Rev. D",
	year = "1976"
}

@article{YanovskyHERCULES,
	author = "V. Yanovsky and others",
	title = "Ultra-{H}igh {I}ntensity-{H}igh {C}ontrast 300-{TW} {L}aser at 0.1{\,H}z {R}epetition {R}ate.",
	journal = "Lasers and Electro-Optics, 2008 and 2008 Conference on Quantum Electronics and Laser Science. CLEO/QELS 2008. Conference on",
	year = "2008"
}

@article{StuartTitan,
	author = "B. C. Stuart and others",
	title = "The {T}itan {L}aser at {LLNL}",
	journal = "Optics InfoBase Conference Papers",
	year = "2006"
}

@article{RankineRHConditions,
	author = "W. J. M. Rankine",
	title = "On the thermodynaimc theory of waves of finite longitudinal disturbances",
	journal = "Philosophical Transactions of the Royal Society of London",
	year = "1870"	
}

@article{HugoniotRHConditions,
	author = "H. Hugoniot",
	title = "M\'{e}moire sur la propagation des mouvements dans les corps et sp\'{e}cialement dans les gaz parfaits",
	journal = "Journal de l'\'{E}cole Polytechnique",
	year = "1887" 
}

@book{SagdeevSagdeevPotential,
	author = "R. Sagdeev",
	title = "Reviews of {P}lasma {P}hysics",
	year = "1966",
	editor = "M. A. Leontovich",
	volumes = "4",
	publisher = "Consultants Bureau",
	location = "New York",
	}

@article{WillingaleFoams,
	author = "L. Willingale and others",
	title  = "Characterization of {H}igh-{I}ntensity {L}aser {P}ropagation in the {R}elativistic {T}ransparent {R}egime through {M}easurement of {E}nergetic {P}roton {B}eams",
	journal = "Phys. Rev. Lett.",
	year = "2009"
}

@article{HookerGemini,
	author = "C. J. Hooker and others",
	title = "Commissioning the Astra Gemini petawatt {T}i:sapphier laser system",
	journal = "Lasers and Electre-Optics, 2008, CLEO 2008",
	year = "2008"
}

@article{CeurvorstChanneling,
    author = "L. Ceurvorst and A. Savin and N. Ratan and M. F. Kasim and J. Sadler and P. A. Norreys and H. Habara and K. A. Tanaka and S. Zhang and M. S. Wei and S. Ivancic and D. H. Froula and W. Theobald",
    title = "Channel optimization og high-intensity laser beams in millimeter-scale plasmas",
    journal = "Phys. Rev. E",
    year = "2018",
    pages = "043208",
    volume = "97"
}

@book{Colvin&Larsen,
    author = "J Colvin and J Larsen",
    title = "Extreme Physics: Properties and Behaviour of Matter at Extreme Conditions",
    publisher = "Cambridge University Press",
    year = "2014",
    pages = "66--69"
}

@article{BataniAblation,
    author = "D. Batani",
    title = "Short-pulse laser ablation of materials at high intensities: Influence of plasma effects",
    journal = "Laser Part. Beams",
    volume = "28",
    pages = "235--244",
    year = "2010"
}

@article{FrantanduonoAblation,
    author = "D. E. Frantanduono and T. R. Boehly and P. M. Celliers and M. A. Barrios and J. H. Eggert and R. F. Smith and D. G. Hicks and G. W. Collins and D. D. Meyerhofer",
    title = "The direct measurement of ablation pressure driven by 351-nm laser radiation",
    journal = "J. Appl. Phys.",
    volume = "110",
    pages = "073110",
    year = "2011"
}

@article{LobetEEEnergy,
    author = "M. Lobet and X. Davoine and D. d'Humi\`eres and L. Gremillet",
    title = "Generation of high-energy electron-positron pairs in the collision of a laser-accelerated electron beam with a multipetawatt laser",
    journal = "Phys. Rev. Accel. Beams",
    volume = "20",
    pages = "043401",
    year = "2017"
}

@article{BreitWheeler,
    author = "G. Breit and J. A. Wheeler",
    title = "Collision of Two Light Quanta",
    journal = "Phys. Rev.",
    volume = "46",
    pages = "1087--1091",
    year = "1934"
}

@article{MeszarosGRB,
    author = "P. M\'esz\'aros",
    title = "Theories of Gamma-Ray Bursts",
    journal = "Annu. Rev. Astron. Astrophys.",
    volume = "40",
    pages = "137--169",
    year = "2002"
}

@article{BetheHeitler,
    author = "H. Bethe and W. Heitler",
    title = "On the Stopping of Fast Particles and on the Creation of Positive Electrons",
    journal = "Proc. R. Soc. A",
    volume = "146",
    pages = "83--112",
    year = "1934"
}

@article{RidgersEPOCHQED,
    author = "C. P. Ridgers and J. G. Kirk and R. Duclous and T. G. Blackburn and C. S. Brady and K. Bennett and T. D. Arber and A. R. Bell",
    title = "Modelling gamma-ray photon emission and pair production in high-intensity laser-matter interactions",
    journal = "J. Comp. Phys.",
    volume = "260",
    pages = "273--285",
    year = "2014"
}

@article{ArberEPOCH,
    author = "T. D. Arber and K. Bennett and C. S. Brady and A. Lawrence-Douglas and M. G. Ramsay and N. J. Sircombe and P. Gillies and R. G. Evans and H. Schmitz and A. R. Bell and C. P. Ridgers",
    title = "Contemporary particle-in-cell approach to laser-plasma modelling",
    journal = "Plasma Phys. Control. Fus.",
    volume = "57",
    pages = "113001",
    year = "2015"
}

@article{GrismayerQEDAbs,
    author = "T. Grismayer and M. Vranic and J. L. Martins and R. A. Fonseca and L. O. Silva",
    title = "Laser absorption via quantum electrodynamics cascades in counter propagating laser pulses",
    journal = "Phys. Plasmas",
    volume = "23",
    pages = "056706",
    year = "2016"
}

@article{VranicCascades,
    author = "M. Vranic and T. Grismayer and R. A. Fonseca and L. O. Silva",
    title = "Electron-positron cascades in multiple-laser optical traps",
    journal = "Plasma Phys. Control. Fus.",
    volume = "59",
    pages = "014040",
    year = "2017"
}

@article{GCasc,
    author = "T. Grismayer and M. Vranic and J. L. Martins and R. A. Fonseca and L. O. Silva",
    title = "Seeded QED cascades in counterpropagating laser pulses",
    journal = "Phys. Rev. E",
    volume = "95",
    pages = "023120",
    year = "2017"
}

@article{ClarkIon,
    author  = "E. L. Clark and K. Krushelnick and J. R. Davies and M. Zepf and M. Tatarakis and F. N. Beg and A. Machacek and P. A. Norreys and M. I. K. Santala and I. Watts and A. E. Dangor",
    title = "Measurements of Energetic Proton Transport through Magnetized Plasma from Intense Laser Interactions with Solids",
    journal = "Phys. Rev. Lett.",
    volume = "84",
    pages = "670",
    year = "2000",
}

@article{DromeyHarm1,
    author = "B. Dromey and M. Zepf and A. Gopal and K. Lancaster and M. S. Wei and K. Krushelnick and M. Tatarakis and N. Vakakis and S. Moustazis and R. Kodama and M. Tampo and C. Stoeckl and R. Clarke and H. Habara and D. Neely and S. Karsch and P. Norreys",
    title = "High harmonic generation in the relativistic limit",
    journal = "Nature Physics",
    volume = "2",
    pages = "456",
    year = "2006"
    }
    
@article{DromeyHarm2,
    author = "B. Dromey and S. kar and C. Bellei and D. C. Carroll and R. J. Clarke and J. S> Green and S. Kneip and K. Markey and S. R. Nagel and P. T. Simpson and L. Willingale and P. McKenna and D. Neely z. Najmudin and K. Krushelnick and P. A. Norreys and M. Zepf",
    title = "Bright Multi-keV Harmonic Generation from Relativistically Oscillating Plasma Surfaces",
    journal = "Phys. Rev. Lett.",
    volume = "99",
    pages = "085001",
    year = "2007"
}

@article{SarriChannels,
    author = "G. Sarri and D. K. Singh and J. R. Davies and F. Fiuza and K. L. Lancaster and E. L. Clark and S. Hassan and J. Jiang and N. Kageiwa and N. Lopes and A. Rehman and C. Russo and R. H. H. Scott and T. Tanimoto and Z. Najmudin and K. A. Tanaka and M. Tatarakis and M. Borghesi and P. A. Norreys",
    title = "Observation of Postsoliton Expansion Following Laser Propagation through an Underdense Plasma",
    journal = "Phys. Rev. Lett.",
    volume = "105",
    pages = "175007",
    year = "2010"
}
